A Search for the $B^0 \to e^+e^-\gamma$ and $B^0 \to \mu^+\mu^-\gamma$ Decays

With the BaBar detector at the PEP-II asymmetric $B$ Factory at SLAC, we present the first search for the decays $B^0\to\ell^+\ell^-\gamma$ ($l=e, \mu$). Using a data set of 292 $fb^{-1}$ collected at the $\Upsilon(4S)$ resonance, we find no significant signal and set the following branching fraction upper limits at 90% confidence level: $\mathcal{B}(B^0\to e^+e^-\gamma)<0.7\times 10^{-7}$ and $\mathcal{B}(B^0\to \mu^+\mu^-\gamma)<3.4\times 10^{-7}$.

==> abstract.tex <==
With the BaBar detector at the PEP-II asymmetric $B$ Factory at SLAC,
we present the first search for the decays
$B^0\rightarrow\ell^+\ell^-\gamma$ ($l=e, \mu$). Using a data set of
292 $fb^{-1}$ collected at the $\Upsilon(4S)$ resonance, we find no
significant signal and set the following branching fraction upper
limits at 90\% confidence level: $\mathcal{B}(B^0\rightarrow
e^+e^-\gamma)<0.7\times 10^{-7}$ and $\mathcal{B}(B^0\rightarrow
\mu^+\mu^-\gamma)<3.4\times 10^{-7}$.


==> dir_B2LLG/babarsym.tex <==
\RequirePackage{xspace}

\newcommand{\ResultE}{0.7\xspace} 
\newcommand{\ResultM}{3.4\xspace} 
\newcommand{\lumi}{292}
\newcommand{\nBB}{320\xspace}

\newcommand{\bllg}{\ensuremath{\Bz \rightarrow \ell^+\ell^-\gamma}\xspace}
\newcommand{\beeg}{\ensuremath{\Bz \rightarrow e^+e^-\gamma}\xspace}
\newcommand{\bmmg}{\ensuremath{\Bz \rightarrow \mu^+\mu^-\gamma}\xspace}
\newcommand{\dE}{\ensuremath{\Delta E}\xspace}
\newcommand{\mes}{\ensuremath{m_{ES}}\xspace}

\newcommand{\effsig}{\ensuremath{\epsilon_{sig}}\xspace}
\newcommand{\nbgexp}{\ensuremath{n_{bg}^{exp}}\xspace}
\newcommand{\nobs}{\ensuremath{n_{obs}}\xspace}

\newcommand{\SigBox}{signal box\xspace}
\newcommand{\SideBox}{sideband area\xspace}
\newcommand{\mDL}{\ensuremath{m_{DL}}\xspace}
\newcommand{\hjCM}{CM\xspace}
\newcommand{\hjfig}{Fig.}
\newcommand{\hjtab}{Table}
\newcommand{\hjeq}{Eq.}
\newcommand{\hjetal}{{\it et al.}}

\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\B       {\ensuremath{B}\xspace}
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}
\def\FourS {\Y4S}
\def\BR         {{\ensuremath{\mathcal{B}}\xspace}}

\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

\def\invfb  {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\pep2{PEP-II}

\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
\newcommand{\nima}      [1]  {\nimBaseA~A~{\bf #1}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}






















